Towards Formal Verification of Password Generation Algorithms used in Password Managers

Password managers are important tools that enable us to use stronger passwords, freeing us from the cognitive burden of remembering them. Despite this, there are still many users who do not fully trust password managers. In this paper, we focus on a feature that most password managers offer that might impact the user's trust, which is the process of generating a random password. We survey which algorithms are most commonly used and we propose a solution for a formally verified reference implementation of a password generation algorithm. We use EasyCrypt as our framework to both specify the reference implementation and to prove its functional correctness and security.

==> algorithm.tex <==

%%% ALGORITHM 1 %%%
\begin{algorithm}
	\caption{RPG Specification} 
	\begin{algorithmic}[1]
	    \Procedure{Generate}{$policies$}
    	    \State $pwLength \leftarrow policies.pwLength$
    	    \State $charSets \leftarrow policies.charSets$
    	    \State $password \leftarrow \varepsilon$
    		\ForAll {$set\in{charSets}$}
    			\For {$i=1,2,\ldots,set.min$}
    				\State $char \leftarrow \textsc{GenerateCharacter}(set)$
    				\State $password \leftarrow password || char$
    			\EndFor
    		\EndFor
    		\While {$len(password) < pwLength$}
    		    \State $availableSets \leftarrow \bigcup_{set\in{charSets}} set$ such that $set.max > 0$
    		    \State $char \leftarrow \textsc{GenerateCharacter}(availableSets)$
    		    \State $password \leftarrow password||char$
    		\EndWhile
    		\State $password \leftarrow \textsc{Permutation}(password)$
    		\State \Return $password$
    	\EndProcedure
    	\State
    	\Procedure{GenerateCharacter}{$set$}
    	\State $choice \leftarrow {RNG}(set.size)$
    	\State $set.max \leftarrow set.max - 1$
    	\State \Return $choice$
    	\EndProcedure
    	\State
        \Procedure{Permutation}{$string$}
            \For {$i=len(string)-1,\ldots,0$}
    		    \State $j \leftarrow {RNG}(i)$
    			\State $aux = string[i]$
    			\State $string[i] = string[j]$
    			\State $string[j] = aux$
    		\EndFor
    		\State \Return $string$
    	\EndProcedure
    	\State
        \Procedure{RNG}{$range$}
	        \State $maxValue \leftarrow (uint64.maxValue / range) * range - 1$
    		\Do
                \State $value \leftarrow$ (uint64) GenerateRandomBytes
            \doWhile{$value > maxValue$}
            \State \Return $value\ \textrm{mod}\ range$
    	\EndProcedure
	\end{algorithmic}
\label{alg:1}
\end{algorithm}
%%% END ALGORITHM 1 %%%

==> original-sec2.tex <==

% SECTION 2
\section{Current Password Generation Algorithms} \label{CurrentPasswordGenerationAlgorithms}
We surveyed the most used algorithms and protocols for generating random passwords of different password managers. We must mention that while some password managers only offered the option of generating a random password, many others offered as well the option of generating a random passphrase (a phrase of a set of words typically separated by a special character). In this paper, we will only focus on ``regular'' passwords because it is still the most common way of user authentication and because while passphrases seem to be an enhancement to usability and maybe to security, it is still not clear if they are indeed better than passwords \cite{keith2009behavioral}.

We surveyed 15 password managers to understand what are the most commonly used protocols, but in this paper we focus on three password managers: Google Chrome's Password Manager (v89.0.4364.1)\footnote{https://source.chromium.org/chromium/chromium/src/+/master:components}, Bitwarden (v1.47.1)\footnote{https://github.com/bitwarden}, and KeePass (v2.46)\footnote{https://github.com/dlech/KeePass2.x}, because they are some of the most used password managers today and also because they are open-source, which allows us to access their source codes and have a deeper understanding of how they generate random passwords.


% SECTION 2.1
\subsection{Policies} \label{Policies}
Password managers are applications for users to generate and store their passwords safely, so typically they expect a user to be interacting with them. However, some password managers have a more ``passive'' role in storing passwords, like Chrome. In this password manager, the user can not arbitrarily ask to generate a new random password. These passwords are generated when a user is registering to a new website automatically. So, sometimes the interface that the password manager offers is not intended for the regular user but for the website that the user is registering to. As these interfaces are identical, from now on we will only mention ``user'' as both the user or the website (unless we want to mention something specific to a website interaction).

Generally the password manager interface allows the user to define some policies regarding the password to be generated. These policies define the structure of the password, meaning that normally they are used to specify the password length, the different sets of characters that may appear on the generated password, the minimum and maximum occurrences of characters of a given set in the password, etc.

These policies are used to strict the space of user-created passwords to preclude easily guessed passwords and thus make passwords more difficult for attackers to guess. While generally speaking this is good for the security of the password, this has the problem of reducing usability. Also, sometimes strict policies can generate some easily guessed passwords (e.g., a policy that enforces the use of lowercase letters, uppercase letters, numbers, and special characters may generate the easily guessed password ``P@ssw0rd'') \cite{shay2016designing}. To prevent these weak passwords to be generated from strict policies, password managers are often equipped with a password strength meter that warns the user about the strength of the password (in our studied password managers, Bitwarden uses zxcvbn \cite{wheeler2016zxcvbn}, KeePass defines their own strength meter, and Chrome does not call any strength meter).

Table \ref{tab:1} shows the different policies the user can specify in the different password managers for the generated password.

%%% TABLE 1 %%%
\begin{table}
\centering
\begin{tabular}{c|c|c|c|}
\cline{2-4}
                                                                                                                                          & \textbf{Chrome}                                                                                                           & \textbf{Bitwarden}                                                                                           & \textbf{KeePass}                                                                                                                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Password\\ Length\end{tabular}}}                                                  & 1-200                                                                                                                     & 5-128                                                                                                        & 1-30000                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{Available sets}}                                                                                             & \begin{tabular}[c]{@{}c@{}}Lowercase Letters\\ Uppercase Letters\\ Alphabetic\\ Numbers\\ Special Characters\end{tabular} & \begin{tabular}[c]{@{}c@{}}Lowercase Letters\\ Uppercase Letters\\ Numbers\\ Special Characters\end{tabular} & \begin{tabular}[c]{@{}c@{}}Lowercase Letters\\ Uppercase Letters\\ Numbers\\ Special Characters\\ Brackets\\ Space\\ Minus\\ Underline\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Define minimum\\ and maximum \\ occurrence of\\ characters per set\end{tabular}}} & Yes                                                                                                                       & \begin{tabular}[c]{@{}c@{}}Yes. Can only\\ define minimum\end{tabular}                                       & No                                                                                                                                                  \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Exclude similar \\ characters\end{tabular}}}                                      & Yes. \{l o I O 0 1\}                                                                                                      & Yes \{l I O 0 1\}                                                                                            & Yes \{l I O 0 1 $|$\}                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Define by hand\\ a character set\end{tabular}}}                                   & No                                                                                                                       & No                                                                                                           & Yes                                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Define by hand\\ a character  set\\ to be excluded\end{tabular}}}                 & No                                                                                                                        & No                                                                                                           & Yes                                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Remove \\ duplicates\end{tabular}}}                                               & No                                                                                                                        & No                                                                                                           & Yes                                                                                                                                                 \\ \hline
\end{tabular}
\medskip
\caption{\label{tab:1}Available options a user can define. The Alphabetic set in Chrome is the union of Lowercase Letters and Uppercase Letters. Special Characters in Chrome and Bitwarden are the set \{- \_ . : !\} while in KeePass it is \{! " \# \$ \% \& ' * + , . / : ; = ? @ \textbackslash \^{} $|$\}. The Brackets set in KeePass is \{( ) \{ \} [ ] < >\}. The Space, Minus, and Underline are the single element sets \{\textvisiblespace\}, \{-\}, and \{\_\} respectively.}
\end{table}
%%% END TABLE 1 %%%


% SECTION 2.2
\subsection{RPG Algorithm} \label{RPGAlgorithm}
Almost all password managers use different algorithms to generate random passwords but we were able to establish some common patterns and methods that were shared between them.

The main idea of these algorithms is to generate random characters from the different character sets until the password length is fulfilled. Notice that when the user changes the policies the only impact on the generation process is that it changes the number of character sets and the characters that belong to those sets (e.g., if we exclude the similar characters we just remove the respective characters from their sets). The only exception is when the user defines the minimum and maximum occurrence of characters per set, which makes the algorithm less trivial. To show how this is achieved, we present the following pseudo-code (Algorithm \ref{alg:1}) which is a generalization of the algorithms of the three password managers, being closely similar to Chrome's algorithm.

%%% ALGORITHM 1 %%%
\begin{algorithm}
	\caption{General Password Generation Algorithm} 
	\begin{algorithmic}[1]
		\Procedure{GeneralGenerate}{$policies$}
    	    \State $pwLength \leftarrow policies.pwLength$
    	    \State $charSets \leftarrow policies.charSets$
    	    \State $password \leftarrow \varepsilon$
    		\ForAll {$set\in{charSets}$}
    			\For {$i=1,2,\ldots,set.min$} \Comment{set.min is the minimum number of characters from that set that must appear on the generated password}
    				\State $char \leftarrow$ Randomly generate a char from the set
    				\State $password \leftarrow password || char$ \Comment{`$||$' is the append operator}
    			\EndFor
    		\EndFor
    		\While {$len(password) < pwLength$}
    		    \State $char \leftarrow$ Randomly generate a char from the union of all sets, while not exceeding the $max$ char occurrence of each set
    		    \State $password \leftarrow password || char$
    		\EndWhile
    		\State Generate a random permutation of $password$
    		\State Output $password$
    	\EndProcedure
	\end{algorithmic}
\label{alg:1}
\end{algorithm}
%%% END ALGORITHM 1 %%%

KeePass's algorithm is simpler, since the user is not able to establish neither the minimum nor the maximum number of occurrences of characters per set. So there is no need to generate  any string permutation, one just needs to define the single set of characters, which is the union of all available sets, and then randomly generate characters from that set.

Regarding Bitwarden, it is basically the same as Chrome. The only difference is that is makes the permutation before generating the characters (i.e., it creates a string like `llluunl' to say that the first three characters are lowercase letters, the following two are uppercase letters, then a number, and finally a lowercase letter. Only then it generates the characters from the respective sets and places them in the respective positions).


% SECTION 2.3
\subsection{String Permutation} \label{StringPermutation}
Given the need to generate a random permutation of the characters of a string, Bitwarden and Chrome both implement an algorithm to do so. The basic idea for both password managers is the same, which is to randomly choose one character from the original string for each position of the new string. This method is described in pseudo-code in Algorithm \ref{alg:2}.

%%% ALGORITHM 2 %%%
\begin{algorithm}
	\caption{String Permutation} 
	\begin{algorithmic}[1]
	    \Procedure{GeneralPermutation}{$string$}
            \For {$i=len(string)-1,\ldots,0$}
    		    \State $j \leftarrow$ Random number between 0 and i
    			\State $aux = string[i]$
    			\State $string[i] = string[j]$
    			\State $string[j] = aux$
    		\EndFor
    	\EndProcedure
	\end{algorithmic}
\label{alg:2}
\end{algorithm}
%%% END ALGORITHM 2 %%%


% SECTION 2.4
\subsection{Random Number Generator} \label{RandomNumberGenerator}
As we can see from Sections \ref{RPGAlgorithm} and \ref{StringPermutation}, the random password generator needs to have some source of randomness to generate the characters and a permutation of them. So, the password generator naturally needs to have an implementation of a Random Number Generator (RNG) that generates random numbers within a range of values, and we want the probability distribution over that range of values to be uniform.

After inspecting the code of the three password managers, we noticed that Chrome and KeePass had an identical RNG, mainly because they generate numbers from 0 to an input \textit{range}. The main idea of these two password managers is to generate random bytes, then casting them to an integer, and then return that value modulo range, so the value it generates is between 0 and range. This is an efficient way to perform this task.

\paragraph*{\textbf{On uniformity and maximum integer values.}}
One must be careful with the approach described above because, since there is a finite maximum value for the random integer (typically integers are 64 bits, so it would be $2^{64}$). This may lead to a non-uniform distribution over the possible values. For example, if the random bytes generated, when cast to an integer, have the maximum possible value of 7 and if range is 5, then a result of 1 would be twice as likely as a result of 3 or 4 (since $1\ \textrm{mod}\ 5 \equiv 6\ \textrm{mod}\ 5 \equiv 1$, while, from 0 to 7, only $3 \equiv 3\ \textrm{mod}\  5$ and $4 \equiv 4\ \textrm{mod}\  5$)

So, some of the possible numbers generated by the random bytes generator must be discarded. This is where Chrome and KeePass slightly differ on their implementation, but they both achieve the same final result.

Chrome's solution to this problem is to find the maximum 64bit unsigned integer \textit{maxValue} such that, given an input \textit{range}, $maxValue\equiv range - 1\ \textrm{mod}\ range$. Then generate random values until you generate a number which is smaller or equal to \textit{maxValue}. Since this value is the maximum value in these conditions, we make sure that there is a high probability of generating a valid number in very few tries.

KeePass's algorithm first generates a random 64bit unsigned integer \textit{value} and then calculates $value\ \textrm{mod}\ range$ (where \textit{range} is again the input). Then, it verifies if the last element of the ``block'' can be generated. By block we mean a sequence of contiguous integers $i,i+1,...,i+range$ such that by applying $\textrm{mod}\ range$ to each element of the sequence, we respectively obtain $0,1,...,range-1$. If the last element can be generated this means that our random number is fine and the algorithm outputs it. If not, it tries again, to avoid the previously mentioned problem of not getting an uniform distribution.

Chrome and KeePass algorithms are described in pseudo-code in Algorithm \ref{alg:3}.

Bitwarden RNG is more complex since it generates numbers from an arbitrary minimum value up to an arbitrary maximum value. Since in our algorithm we will only need to generate numbers from 0 to any given maximum value, the simpler implementations of Chrome and KeePass are sufficient for us to focus on.

%%% ALGORITHM 3 %%%
\begin{algorithm}
	\caption{RNGs with maximum range} 
	\begin{algorithmic}[1]
	    \Procedure{ChromeRNG}{$range$}
	        \State $maxValue \leftarrow (uint64.maxValue / range) * range - 1$ \Comment{uint64.maxValue is the maximum value an unsigned integer with 64 bits can take; `/' is the Euclidean division}
    		\Do
                \State $value \leftarrow$ (uint64) GenerateRandomBytes
            \doWhile{$value > maxValue$}
            \State \Return $value\ \textrm{mod}\ range$
    	\EndProcedure
    	\State
    	\State
	    \Procedure{KeePassRNG}{$range$}
    		\Do
                \State $genValue \leftarrow$ (uint64) GenerateRandomBytes
                \State $value \leftarrow genValue\ \textrm{mod}\ range$
            \doWhile{$(genValue - value) > (uint64.maxValue - (range - 1))$}
            \State \Return $value$
    	\EndProcedure
	\end{algorithmic}
\label{alg:3}
\end{algorithm}
%%% END ALGORITHM 3 %%%


% SECTION 2.5
\subsection{Random Bytes Generator} \label{RandomBytesGenerator}
At the bottom of these implementations there is a random bytes generator. Regarding this, the three password managers considered had different approaches. Chrome uses different system calls based on the operating system the password manager is running, Bitwarden uses NodeJS \textit{randomBytes()} method, while KeePass defines their own random bytes generator based on ChaCha20.

We did not explore this feature in depth, because we think it is not necessary and we leave it as future work. However, depending on the project development, we might explore this and try to define our own random bytes generator and verify it.
For now, we assume that these random bytes generators exist and are secure.


